Focus On What Matters: Separated Models For Visual-Based RL Generalization

A primary challenge for visual-based Reinforcement Learning (RL) is to generalize effectively across unseen environments. Although previous studies have explored different auxiliary tasks to enhance generalization, few adopt image reconstruction due to concerns about exacerbating overfitting to task-irrelevant features during training. Perceiving the pre-eminence of image reconstruction in representation learning, we propose SMG (Separated Models for Generalization), a novel approach that exploits image reconstruction for generalization. SMG introduces two model branches to extract task-relevant and task-irrelevant representations separately from visual observations via cooperatively reconstruction. Built upon this architecture, we further emphasize the importance of task-relevant features for generalization. Specifically, SMG incorporates two additional consistency losses to guide the agent's focus toward task-relevant areas across different scenarios, thereby achieving free from overfitting. Extensive experiments in DMC demonstrate the SOTA performance of SMG in generalization, particularly excelling in video-background settings. Evaluations on robotic manipulation tasks further confirm the robustness of SMG in real-world applications.

==> tables/ablations.tex <==

\begin{table}[t]
    \label{tab:ablations}
    \vspace{0.075in}
    \centering
    \resizebox{\tablesize\textwidth}{!}{%
    \begin{tabular}{cccccccc}
    \toprule
    
    \bf{DMControl}       & SMG   &w/o $L_{\text{mask}}$&w/o $L_{\text{action}}$&w/o $L_{\text{fore\_consist}}$&w/o $L_{\text{q\_consist}}$&w/o $L_{\text{back}}$     \\
    (video hard)         & (raw) &&&&& \\
    
    \midrule
    \texttt{cartpole,}        & $764\pm32$ & $590\pm84$ & $631\pm92$ & $720\pm100$ & $238\pm82$ & $763\pm44$ \vspace{-0.75ex} \\    \texttt{swingup}        
                          & 
                          & \best{$\scriptstyle{-23\%}$}
                          & \best{$\scriptstyle{-17\%}$}
                          & \best{$\scriptstyle{-6\%}$}
                          & \best{$\scriptstyle{-69\%}$}
                          & \best{$\scriptstyle{0\%}$} \vspace{0.75ex} \\

    \texttt{finger,}        & $910\pm61$ & $731\pm130$ & $609\pm352$ & $695\pm103$ & $434\pm189$ & $412\pm170$ \vspace{-0.75ex} \\    \texttt{spin}        
                          & 
                          & \best{$\scriptstyle{-20\%}$}
                          & \best{$\scriptstyle{-33\%}$}
                          & \best{$\scriptstyle{-24\%}$}
                          & \best{$\scriptstyle{-52\%}$}
                          & \best{$\scriptstyle{-55\%}$} \vspace{0.75ex} \\

    \texttt{walker,}        & $939\pm16$ & $836\pm127$ & $855\pm96$ & $885\pm45$ & $392\pm163$ & $775\pm144$ \vspace{-0.75ex} \\    \texttt{stand}        
                          & 
                          & \best{$\scriptstyle{-11\%}$}
                          & \best{$\scriptstyle{-9\%}$}
                          & \best{$\scriptstyle{-6\%}$}
                          & \best{$\scriptstyle{-58\%}$}
                          & \best{$\scriptstyle{-17\%}$} \vspace{0.75ex} \\

    \texttt{walker,}        & $736\pm36$ & $416\pm98$ & $670\pm22$ & $642\pm63$ & $217\pm103$ & $657\pm103$ \vspace{-0.75ex} \\    \texttt{walk}        
                          & 
                          & \best{$\scriptstyle{-43\%}$}
                          & \best{$\scriptstyle{-9\%}$}
                          & \best{$\scriptstyle{-13\%}$}
                          & \best{$\scriptstyle{-71\%}$}
                          & \best{$\scriptstyle{-11\%}$} \vspace{0.75ex} \\

    \texttt{cheetah,}        & $303\pm46$ & $162\pm100$ & $212\pm52$ & $247\pm40$ & $130\pm37$ & $233\pm110$ \vspace{-0.75ex} \\    \texttt{run}        
                          & 
                          & \best{$\scriptstyle{-47\%}$}
                          & \best{$\scriptstyle{-30\%}$}
                          & \best{$\scriptstyle{-18\%}$}
                          & \best{$\scriptstyle{-57\%}$}
                          & \best{$\scriptstyle{-23\%}$} \vspace{0.75ex} \\

    \midrule
\vspace{0.05in}
    \bf{Average}        & & \best{$-29\%$} & \best{$-20\%$} & \best{$-13\%$} & \best{$-61\%$} & \best{$-21\%$} \vspace{-0.75ex} \\

    \bottomrule
    \end{tabular}
    }
    \vspace{0.1in}
    \caption{video hard. \best{Red} indicates the best and \second{blue} indicates the second best. $\Delta=$ improvement of \dino over the second best.}
\end{table}

==> tables/ablations_color_easy.tex <==

\begin{table}[h]
    \label{tab:ablations}
    \vspace{0.075in}
    \centering
    \resizebox{0.9\textwidth}{!}{%
    \begin{tabular}{cccccccc}
    \toprule
    
    \bf{DMControl}       & SMG   &w/o $L_{\text{fore\_consis}}$&w/o $L_{\text{action}}$&w/o $L_{\text{back}}$&w/o $L_{\text{mask}}$&w/o $L_{\text{q\_consis}}$     \\

    (color easy)         & (full) &&&&& \\
    
    \midrule
    \texttt{cartpole,}        & $854\pm13$ & $769\pm60$ & $811\pm29$ & $811\pm58$ & $844\pm10$ & $791\pm53$ \vspace{-0.75ex} \\    \texttt{swingup}        
                          & 
                          & \best{$\scriptstyle{-85\:(10\%)}$}
                          & \best{$\scriptstyle{-43\:(5\%)}$}
                          & \best{$\scriptstyle{-43\:(5\%)}$}
                          & \best{$\scriptstyle{-10\:(1\%)}$}
                          & \best{$\scriptstyle{-63\:(7\%)}$} \vspace{0.75ex} \\

    \texttt{finger,}        & $957\pm52$ & $870\pm157$ & $863\pm82$ & $703\pm178$ & $913\pm28$ & $867\pm76$ \vspace{-0.75ex} \\    \texttt{spin}        
                          & 
                          & \best{$\scriptstyle{-87\:(9\%)}$}
                          & \best{$\scriptstyle{-94\:(10\%)}$}
                          & \best{$\scriptstyle{-254\:(27\%)}$}
                          & \best{$\scriptstyle{-44\:(5\%)}$}
                          & \best{$\scriptstyle{-90\:(9\%)}$} \vspace{0.75ex} \\

    \texttt{walker,}        & $965\pm13$ & $895\pm74$ & $868\pm84$ & $956\pm19$ & $946\pm27$ & $687\pm397$ \vspace{-0.75ex} \\    \texttt{stand}        
                          & 
                          & \best{$\scriptstyle{-70\:(7\%)}$}
                          & \best{$\scriptstyle{-97\:(10\%)}$}
                          & \best{$\scriptstyle{-9\:(1\%)}$}
                          & \best{$\scriptstyle{-19\:(2\%)}$}
                          & \best{$\scriptstyle{-278\:(29\%)}$} \vspace{0.75ex} \\

    \texttt{walker,}        & $842\pm76$ & $779\pm42$ & $791\pm108$ & $814\pm51$ & $787\pm128$ & $745\pm115$ \vspace{-0.75ex} \\    \texttt{walk}        
                          & 
                          & \best{$\scriptstyle{-63\:(7\%)}$}
                          & \best{$\scriptstyle{-51\:(6\%)}$}
                          & \best{$\scriptstyle{-28\:(3\%)}$}
                          & \best{$\scriptstyle{-55\:(7\%)}$}
                          & \best{$\scriptstyle{-97\:(12\%)}$} \vspace{0.75ex} \\

    \texttt{cheetah,}        & $346\pm27$ & $310\pm35$ & $346\pm80$ & $269\pm51$ & $365\pm62$ & $290\pm46$ \vspace{-0.75ex} \\    \texttt{run}        
                          & 
                          & \best{$\scriptstyle{-36\:(10\%)}$}
                          & \best{$\scriptstyle{0\:(0\%)}$}
                          & \best{$\scriptstyle{-77\:(22\%)}$}
                          & \best{$\scriptstyle{19\:(5\%)}$}
                          & \best{$\scriptstyle{-56\:(16\%)}$} \vspace{0.75ex} \\

    \midrule
\vspace{0.05in}
    \bf{Average}        & & \best{$-9\%$} & \best{$-6\%$} & \best{$-12\%$} & \best{$-2\%$} & \best{$-15\%$} \vspace{-0.75ex} \\

    \bottomrule
    \end{tabular}
    }
    \vspace{0.1in}
    \caption{Ablation study in DMControl-GB (\textit{video-hard}). \best{Red} indicates the performance drop of the ablated model compared to the full model.}
\end{table}

==> tables/ablations_color_hard.tex <==

\begin{table}[h]
    \label{tab:ablations}
    \vspace{0.075in}
    \centering
    \resizebox{0.9\textwidth}{!}{%
    \begin{tabular}{cccccccc}
    \toprule
    
    \bf{DMControl}       & SMG   &w/o $L_{\text{fore\_consis}}$&w/o $L_{\text{action}}$&w/o $L_{\text{back}}$&w/o $L_{\text{mask}}$&w/o $L_{\text{q\_consis}}$     \\

    (color hard)         & (full) &&&&& \\
    
    \midrule
    \texttt{cartpole,}        & $726\pm62$ & $770\pm53$ & $753\pm76$ & $753\pm40$ & $712\pm97$ & $670\pm30$ \vspace{-0.75ex} \\    \texttt{swingup}        
                          & 
                          & \best{$\scriptstyle{44\:(6\%)}$}
                          & \best{$\scriptstyle{27\:(4\%)}$}
                          & \best{$\scriptstyle{27\:(4\%)}$}
                          & \best{$\scriptstyle{-14\:(2\%)}$}
                          & \best{$\scriptstyle{-56\:(8\%)}$} \vspace{0.75ex} \\

    \texttt{finger,}        & $841\pm113$ & $794\pm140$ & $759\pm178$ & $675\pm172$ & $848\pm64$ & $715\pm154$ \vspace{-0.75ex} \\    \texttt{spin}        
                          & 
                          & \best{$\scriptstyle{-47\:(6\%)}$}
                          & \best{$\scriptstyle{-82\:(10\%)}$}
                          & \best{$\scriptstyle{-166\:(20\%)}$}
                          & \best{$\scriptstyle{7\:(1\%)}$}
                          & \best{$\scriptstyle{-126\:(15\%)}$} \vspace{0.75ex} \\

    \texttt{walker,}        & $878\pm70$ & $916\pm45$ & $859\pm118$ & $946\pm11$ & $954\pm3$ & $488\pm274$ \vspace{-0.75ex} \\    \texttt{stand}        
                          & 
                          & \best{$\scriptstyle{38\:(4\%)}$}
                          & \best{$\scriptstyle{-19\:(2\%)}$}
                          & \best{$\scriptstyle{68\:(8\%)}$}
                          & \best{$\scriptstyle{76\:(9\%)}$}
                          & \best{$\scriptstyle{-390\:(44\%)}$} \vspace{0.75ex} \\

    \texttt{walker,}        & $719\pm114$ & $687\pm63$ & $698\pm74$ & $608\pm59$ & $715\pm78$ & $427\pm24$ \vspace{-0.75ex} \\    \texttt{walk}        
                          & 
                          & \best{$\scriptstyle{-32\:(4\%)}$}
                          & \best{$\scriptstyle{-21\:(3\%)}$}
                          & \best{$\scriptstyle{-111\:(15\%)}$}
                          & \best{$\scriptstyle{-4\:(1\%)}$}
                          & \best{$\scriptstyle{-292\:(41\%)}$} \vspace{0.75ex} \\

    \texttt{cheetah,}        & $299\pm22$ & $309\pm22$ & $335\pm31$ & $259\pm85$ & $319\pm26$ & $163\pm15$ \vspace{-0.75ex} \\    \texttt{run}        
                          & 
                          & \best{$\scriptstyle{10\:(3\%)}$}
                          & \best{$\scriptstyle{36\:(12\%)}$}
                          & \best{$\scriptstyle{-40\:(13\%)}$}
                          & \best{$\scriptstyle{20\:(7\%)}$}
                          & \best{$\scriptstyle{-136\:(45\%)}$} \vspace{0.75ex} \\

    \midrule
\vspace{0.05in}
    \bf{Average}        & & \best{$1\%$} & \best{$0\%$} & \best{$-7\%$} & \best{$3\%$} & \best{$-31\%$} \vspace{-0.75ex} \\

    \bottomrule
    \end{tabular}
    }
    \vspace{0.1in}
    \caption{Ablation study in DMControl-GB (\textit{video-hard}). \best{Red} indicates the performance drop of the ablated model compared to the full model.}
\end{table}

==> tables/ablations_train.tex <==

\begin{table}[h]
    \label{tab:ablations}
    \vspace{0.075in}
    \centering
    \resizebox{0.9\textwidth}{!}{%
    \begin{tabular}{cccccccc}
    \toprule
    
    \bf{DMControl}       & SMG   &w/o $L_{\text{fore\_consis}}$&w/o $L_{\text{action}}$&w/o $L_{\text{back}}$&w/o $L_{\text{mask}}$&w/o $L_{\text{q\_consis}}$     \\

    (train)         & (full) &&&&& \\
    
    \midrule
    \texttt{cartpole,}        & $858\pm9$ & $805\pm39$ & $833\pm15$ & $836\pm25$ & $849\pm1$ & $850\pm2$ \vspace{-0.75ex} \\    \texttt{swingup}        
                          & 
                          & \best{$\scriptstyle{-53\:(6\%)}$}
                          & \best{$\scriptstyle{-25\:(3\%)}$}
                          & \best{$\scriptstyle{-22\:(3\%)}$}
                          & \best{$\scriptstyle{-9\:(1\%)}$}
                          & \best{$\scriptstyle{-8\:(1\%)}$} \vspace{0.75ex} \\

    \texttt{finger,}        & $961\pm44$ & $870\pm150$ & $943\pm57$ & $725\pm188$ & $933\pm49$ & $944\pm55$ \vspace{-0.75ex} \\    \texttt{spin}        
                          & 
                          & \best{$\scriptstyle{-91\:(9\%)}$}
                          & \best{$\scriptstyle{-18\:(2\%)}$}
                          & \best{$\scriptstyle{-236\:(25\%)}$}
                          & \best{$\scriptstyle{-28\:(3\%)}$}
                          & \best{$\scriptstyle{-17\:(2\%)}$} \vspace{0.75ex} \\

    \texttt{walker,}        & $964\pm18$ & $951\pm7$ & $892\pm92$ & $958\pm14$ & $959\pm4$ & $689\pm401$ \vspace{-0.75ex} \\    \texttt{stand}        
                          & 
                          & \best{$\scriptstyle{-13\:(1\%)}$}
                          & \best{$\scriptstyle{-72\:(7\%)}$}
                          & \best{$\scriptstyle{-6\:(1\%)}$}
                          & \best{$\scriptstyle{-5\:(1\%)}$}
                          & \best{$\scriptstyle{-275\:(29\%)}$} \vspace{0.75ex} \\

    \texttt{walker,}        & $846\pm86$ & $775\pm51$ & $819\pm91$ & $861\pm26$ & $826\pm90$ & $913\pm28$ \vspace{-0.75ex} \\    \texttt{walk}        
                          & 
                          & \best{$\scriptstyle{-71\:(8\%)}$}
                          & \best{$\scriptstyle{-27\:(3\%)}$}
                          & \best{$\scriptstyle{15\:(2\%)}$}
                          & \best{$\scriptstyle{-20\:(2\%)}$}
                          & \best{$\scriptstyle{67\:(8\%)}$} \vspace{0.75ex} \\

    \texttt{cheetah,}        & $357\pm25$ & $330\pm23$ & $376\pm51$ & $307\pm78$ & $384\pm39$ & $429\pm62$ \vspace{-0.75ex} \\    \texttt{run}        
                          & 
                          & \best{$\scriptstyle{-27\:(8\%)}$}
                          & \best{$\scriptstyle{19\:(5\%)}$}
                          & \best{$\scriptstyle{-50\:(14\%)}$}
                          & \best{$\scriptstyle{27\:(8\%)}$}
                          & \best{$\scriptstyle{72\:(20\%)}$} \vspace{0.75ex} \\

    \midrule
\vspace{0.05in}
    \bf{Average}        & & \best{$-6\%$} & \best{$-2\%$} & \best{$-8\%$} & \best{$0\%$} & \best{$-1\%$} \vspace{-0.75ex} \\

    \bottomrule
    \end{tabular}
    }
    \vspace{0.1in}
    \caption{Ablation study in DMControl-GB (\textit{video-hard}). \best{Red} indicates the performance drop of the ablated model compared to the full model.}
\end{table}

==> tables/ablations_video_easy.tex <==

\begin{table}[h]
    \label{tab:ablations}
    \vspace{0.075in}
    \centering
    \resizebox{0.9\textwidth}{!}{%
    \begin{tabular}{cccccccc}
    \toprule
    
    \bf{DMControl}       & SMG   &w/o $L_{\text{fore\_consis}}$&w/o $L_{\text{action}}$&w/o $L_{\text{back}}$&w/o $L_{\text{mask}}$&w/o $L_{\text{q\_consis}}$     \\

    (video easy)         & (full) &&&&& \\
    
    \midrule
    \texttt{cartpole,}        & $839\pm16$ & $752\pm53$ & $781\pm16$ & $811\pm19$ & $795\pm56$ & $615\pm81$ \vspace{-0.75ex} \\    \texttt{swingup}        
                          & 
                          & \best{$\scriptstyle{-87\:(10\%)}$}
                          & \best{$\scriptstyle{-58\:(7\%)}$}
                          & \best{$\scriptstyle{-28\:(3\%)}$}
                          & \best{$\scriptstyle{-44\:(5\%)}$}
                          & \best{$\scriptstyle{-224\:(27\%)}$} \vspace{0.75ex} \\

    \texttt{finger,}        & $952\pm48$ & $848\pm139$ & $783\pm228$ & $687\pm181$ & $906\pm51$ & $830\pm65$ \vspace{-0.75ex} \\    \texttt{spin}        
                          & 
                          & \best{$\scriptstyle{-104\:(11\%)}$}
                          & \best{$\scriptstyle{-169\:(18\%)}$}
                          & \best{$\scriptstyle{-265\:(28\%)}$}
                          & \best{$\scriptstyle{-46\:(5\%)}$}
                          & \best{$\scriptstyle{-122\:(13\%)}$} \vspace{0.75ex} \\

    \texttt{walker,}        & $961\pm19$ & $944\pm9$ & $896\pm93$ & $942\pm12$ & $953\pm4$ & $692\pm404$ \vspace{-0.75ex} \\    \texttt{stand}        
                          & 
                          & \best{$\scriptstyle{-17\:(2\%)}$}
                          & \best{$\scriptstyle{-65\:(7\%)}$}
                          & \best{$\scriptstyle{-19\:(2\%)}$}
                          & \best{$\scriptstyle{-8\:(1\%)}$}
                          & \best{$\scriptstyle{-269\:(28\%)}$} \vspace{0.75ex} \\

    \texttt{walker,}        & $828\pm57$ & $751\pm13$ & $805\pm70$ & $839\pm27$ & $721\pm30$ & $696\pm33$ \vspace{-0.75ex} \\    \texttt{walk}        
                          & 
                          & \best{$\scriptstyle{-77\:(9\%)}$}
                          & \best{$\scriptstyle{-23\:(3\%)}$}
                          & \best{$\scriptstyle{11\:(1\%)}$}
                          & \best{$\scriptstyle{-107\:(13\%)}$}
                          & \best{$\scriptstyle{-132\:(16\%)}$} \vspace{0.75ex} \\

    \texttt{cheetah,}        & $348\pm28$ & $322\pm25$ & $357\pm63$ & $284\pm83$ & $367\pm21$ & $334\pm36$ \vspace{-0.75ex} \\    \texttt{run}        
                          & 
                          & \best{$\scriptstyle{-26\:(7\%)}$}
                          & \best{$\scriptstyle{9\:(3\%)}$}
                          & \best{$\scriptstyle{-64\:(18\%)}$}
                          & \best{$\scriptstyle{19\:(5\%)}$}
                          & \best{$\scriptstyle{-14\:(4\%)}$} \vspace{0.75ex} \\

    \midrule
\vspace{0.05in}
    \bf{Average}        & & \best{$-8\%$} & \best{$-6\%$} & \best{$-10\%$} & \best{$-4\%$} & \best{$-18\%$} \vspace{-0.75ex} \\

    \bottomrule
    \end{tabular}
    }
    \vspace{0.1in}
    \caption{Ablation study in DMControl-GB (\textit{video-hard}). \best{Red} indicates the performance drop of the ablated model compared to the full model.}
\end{table}

==> tables/dmc-gb-average.tex <==

\begin{table}[t]
    \label{tab:dmc-all}
    \vspace{0.075in}
    \centering
    \resizebox{\tablesize\textwidth}{!}{%
    \begin{tabular}{cccccccccc}
    \toprule
    
    \bf{DMControl-GB}      & SAC & DrQ & SODA & SVEA    & SRM & SGQN & \textbf{SMG} & $\Delta$ \\
    (average)           &     &     &  &(overlay) &  (SAC) &   & (ours)       &          \\
    
    \midrule

    \texttt{cartpole,}        & $176$ & $642$ & $591$ & \second{\bf{720}} & $676$ & $704$ & \best{\bf{808}} & $+88$ \vspace{-0.75ex} \\    \texttt{swingup}        
                          & $\scriptstyle{\pm11}$
                          & $\scriptstyle{\pm255}$
                          & $\scriptstyle{\pm132}$
                          & \second{$\scriptstyle{\pm110}$}
                          & $\scriptstyle{\pm226}$
                          & $\scriptstyle{\pm77}$
                          & \best{$\scriptstyle{\pm53}$}
                          & $\scriptstyle{12\%}$ \vspace{0.75ex} \\

    \texttt{finger,}        & $213$ & $586$ & $630$ & $776$ & $690$ & \second{\bf{809}} & \best{\bf{924}} & $+115$ \vspace{-0.75ex} \\    \texttt{spin}        
                          & $\scriptstyle{\pm107}$
                          & $\scriptstyle{\pm297}$
                          & $\scriptstyle{\pm173}$
                          & $\scriptstyle{\pm215}$
                          & $\scriptstyle{\pm297}$
                          & \second{$\scriptstyle{\pm88}$}
                          & \best{$\scriptstyle{\pm45}$}
                          & $\scriptstyle{14\%}$ \vspace{0.75ex} \\

    \texttt{walker,}        & $489$ & $747$ & $772$ & $891$ & $845$ & \second{\bf{893}} & \best{\bf{945}} & $+52$ \vspace{-0.75ex} \\    \texttt{stand}        
                          & $\scriptstyle{\pm147}$
                          & $\scriptstyle{\pm243}$
                          & $\scriptstyle{\pm198}$
                          & $\scriptstyle{\pm70}$
                          & $\scriptstyle{\pm154}$
                          & \second{$\scriptstyle{\pm61}$}
                          & \best{$\scriptstyle{\pm33}$}
                          & $\scriptstyle{6\%}$ \vspace{0.75ex} \\

    \texttt{walker,}        & $338$ & $556$ & $442$ & $614$ & $531$ & \second{\bf{755}} & \best{\bf{859}} & $+104$ \vspace{-0.75ex} \\    \texttt{walk}        
                          & $\scriptstyle{\pm109}$
                          & $\scriptstyle{\pm254}$
                          & $\scriptstyle{\pm147}$
                          & $\scriptstyle{\pm146}$
                          & $\scriptstyle{\pm199}$
                          & \second{$\scriptstyle{\pm103}$}
                          & \best{$\scriptstyle{\pm72}$}
                          & $\scriptstyle{14\%}$ \vspace{0.75ex} \\

    \texttt{cheetah,}        & $201$ & $199$ & $195$ & $242$ & $223$ & \second{\bf{262}} & \best{\bf{331}} & $+69$ \vspace{-0.75ex} \\    \texttt{run}        
                          & $\scriptstyle{\pm85}$
                          & $\scriptstyle{\pm100}$
                          & $\scriptstyle{\pm40}$
                          & $\scriptstyle{\pm72}$
                          & $\scriptstyle{\pm75}$
                          & \second{$\scriptstyle{\pm77}$}
                          & \best{$\scriptstyle{\pm24}$}
                          & $\scriptstyle{26\%}$ \vspace{0.75ex} \\



    \bottomrule
    \end{tabular}
    }
    \vspace{0.1in}
    \caption{average. \best{Red} indicates the best and \second{blue} indicates the second best. $\Delta=$ improvement of \dino over the second best.}
\end{table}

==> tables/dmc-gb-color-easy.tex <==

\begin{table}[t]
    \label{tab:dmc-all}
    \vspace{0.075in}
    \centering
    \resizebox{\tablesize\textwidth}{!}{%
    \begin{tabular}{cccccccccc}
    \toprule
    
    \bf{DMControl-GB}      & SAC & DrQ & SODA & SVEA    & SRM & SGQN & \textbf{SMG} & $\Delta$ \\
    (color easy)           &     &     &  &(overlay) &  (SAC) &   & (ours)       &          \\
    
    \midrule

    \texttt{cartpole,}        & $178$ & $845$ & $720$ & $809$ & \best{\bf{856}} & $764$ & \second{\bf{854}} & $-2$ \vspace{-0.75ex} \\    \texttt{swingup}        
                          & $\scriptstyle{\pm24}$
                          & $\scriptstyle{\pm29}$
                          & $\scriptstyle{\pm109}$
                          & $\scriptstyle{\pm40}$
                          & \best{$\scriptstyle{\pm14}$}
                          & $\scriptstyle{\pm84}$
                          & \second{$\scriptstyle{\pm13}$}
                          & $\scriptstyle{0\%}$ \vspace{0.75ex} \\

    \texttt{finger,}        & $296$ & $827$ & $761$ & \second{\bf{919}} & $916$ & $852$ & \best{\bf{957}} & $+38$ \vspace{-0.75ex} \\    \texttt{spin}        
                          & $\scriptstyle{\pm22}$
                          & $\scriptstyle{\pm174}$
                          & $\scriptstyle{\pm87}$
                          & \second{$\scriptstyle{\pm43}$}
                          & $\scriptstyle{\pm34}$
                          & $\scriptstyle{\pm126}$
                          & \best{$\scriptstyle{\pm52}$}
                          & $\scriptstyle{4\%}$ \vspace{0.75ex} \\

    \texttt{walker,}        & $592$ & $827$ & $929$ & \second{\bf{957}} & $953$ & $906$ & \best{\bf{965}} & $+8$ \vspace{-0.75ex} \\    \texttt{stand}        
                          & $\scriptstyle{\pm274}$
                          & $\scriptstyle{\pm97}$
                          & $\scriptstyle{\pm23}$
                          & \second{$\scriptstyle{\pm4}$}
                          & $\scriptstyle{\pm5}$
                          & $\scriptstyle{\pm50}$
                          & \best{$\scriptstyle{\pm13}$}
                          & $\scriptstyle{1\%}$ \vspace{0.75ex} \\

    \texttt{walker,}        & $430$ & $669$ & $539$ & $705$ & $632$ & \second{\bf{805}} & \best{\bf{915}} & $+110$ \vspace{-0.75ex} \\    \texttt{walk}        
                          & $\scriptstyle{\pm33}$
                          & $\scriptstyle{\pm68}$
                          & $\scriptstyle{\pm51}$
                          & $\scriptstyle{\pm124}$
                          & $\scriptstyle{\pm93}$
                          & \second{$\scriptstyle{\pm47}$}
                          & \best{$\scriptstyle{\pm36}$}
                          & $\scriptstyle{14\%}$ \vspace{0.75ex} \\

    \texttt{cheetah,}        & $253$ & $237$ & $219$ & $289$ & $272$ & \second{\bf{312}} & \best{\bf{346}} & $+34$ \vspace{-0.75ex} \\    \texttt{run}        
                          & $\scriptstyle{\pm27}$
                          & $\scriptstyle{\pm74}$
                          & $\scriptstyle{\pm46}$
                          & $\scriptstyle{\pm43}$
                          & $\scriptstyle{\pm24}$
                          & \second{$\scriptstyle{\pm34}$}
                          & \best{$\scriptstyle{\pm27}$}
                          & $\scriptstyle{11\%}$ \vspace{0.75ex} \\



    \bottomrule
    \end{tabular}
    }
    \vspace{0.1in}
    \caption{color easy. \best{Red} indicates the best and \second{blue} indicates the second best. $\Delta=$ improvement of \dino over the second best.}
\end{table}

==> tables/dmc-gb-color-hard.tex <==

\begin{table}[t]
    \label{tab:dmc-all}
    \vspace{0.075in}
    \centering
    \resizebox{\tablesize\textwidth}{!}{%
    \begin{tabular}{cccccccccc}
    \toprule
    
    \bf{DMControl-GB}      & SAC & DrQ & SODA & SVEA    & SRM & SGQN & \textbf{SMG} & $\Delta$ \\
    (color hard)           &     &     &  &(overlay) &  (SAC) &   & (ours)       &          \\
    
    \midrule

    \texttt{cartpole,}        & $184$ & $717$ & $585$ & \best{\bf{752}} & \second{\bf{752}} & $636$ & $726$ & $-26$ \vspace{-0.75ex} \\    \texttt{swingup}        
                          & $\scriptstyle{\pm26}$
                          & $\scriptstyle{\pm133}$
                          & $\scriptstyle{\pm66}$
                          & \best{$\scriptstyle{\pm86}$}
                          & \second{$\scriptstyle{\pm103}$}
                          & $\scriptstyle{\pm110}$
                          & $\scriptstyle{\pm62}$
                          & $\scriptstyle{3\%}$ \vspace{0.75ex} \\

    \texttt{finger,}        & $271$ & $655$ & $663$ & \best{\bf{868}} & $834$ & $700$ & \second{\bf{841}} & $-27$ \vspace{-0.75ex} \\    \texttt{spin}        
                          & $\scriptstyle{\pm23}$
                          & $\scriptstyle{\pm214}$
                          & $\scriptstyle{\pm106}$
                          & \best{$\scriptstyle{\pm74}$}
                          & $\scriptstyle{\pm90}$
                          & $\scriptstyle{\pm219}$
                          & \second{$\scriptstyle{\pm113}$}
                          & $\scriptstyle{3\%}$ \vspace{0.75ex} \\

    \texttt{walker,}        & $526$ & $769$ & $719$ & $799$ & \second{\bf{807}} & $788$ & \best{\bf{878}} & $+71$ \vspace{-0.75ex} \\    \texttt{stand}        
                          & $\scriptstyle{\pm259}$
                          & $\scriptstyle{\pm182}$
                          & $\scriptstyle{\pm138}$
                          & $\scriptstyle{\pm118}$
                          & \second{$\scriptstyle{\pm128}$}
                          & $\scriptstyle{\pm114}$
                          & \best{$\scriptstyle{\pm70}$}
                          & $\scriptstyle{9\%}$ \vspace{0.75ex} \\

    \texttt{walker,}        & $379$ & $456$ & $396$ & $571$ & $483$ & \second{\bf{632}} & \best{\bf{739}} & $+107$ \vspace{-0.75ex} \\    \texttt{walk}        
                          & $\scriptstyle{\pm37}$
                          & $\scriptstyle{\pm192}$
                          & $\scriptstyle{\pm78}$
                          & $\scriptstyle{\pm134}$
                          & $\scriptstyle{\pm123}$
                          & \second{$\scriptstyle{\pm176}$}
                          & \best{$\scriptstyle{\pm31}$}
                          & $\scriptstyle{17\%}$ \vspace{0.75ex} \\

    \texttt{cheetah,}        & $208$ & $147$ & $199$ & \second{\bf{238}} & $203$ & $210$ & \best{\bf{299}} & $+61$ \vspace{-0.75ex} \\    \texttt{run}        
                          & $\scriptstyle{\pm54}$
                          & $\scriptstyle{\pm80}$
                          & $\scriptstyle{\pm38}$
                          & \second{$\scriptstyle{\pm69}$}
                          & $\scriptstyle{\pm30}$
                          & $\scriptstyle{\pm18}$
                          & \best{$\scriptstyle{\pm22}$}
                          & $\scriptstyle{26\%}$ \vspace{0.75ex} \\



    \bottomrule
    \end{tabular}
    }
    \vspace{0.1in}
    \caption{color hard. \best{Red} indicates the best and \second{blue} indicates the second best. $\Delta=$ improvement of \dino over the second best.}
\end{table}

==> tables/dmc-gb-train.tex <==

\begin{table}[t]
    \label{tab:dmc-all}
    \vspace{0.075in}
    \centering
    \resizebox{\tablesize\textwidth}{!}{%
    \begin{tabular}{cccccccccc}
    \toprule
    
    \bf{DMControl-GB}      & SAC & DrQ & SODA & SVEA    & SRM & SGQN & \textbf{SMG} & $\Delta$ \\
    (train)           &     &     &  &(overlay) &  (SAC) &   & (ours)       &          \\
    
    \midrule

    \texttt{cartpole,}        & $186$ & \best{\bf{872}} & $687$ & $809$ & \second{\bf{871}} & $805$ & $858$ & $-14$ \vspace{-0.75ex} \\    \texttt{swingup}        
                          & $\scriptstyle{\pm6}$
                          & \best{$\scriptstyle{\pm10}$}
                          & $\scriptstyle{\pm175}$
                          & $\scriptstyle{\pm42}$
                          & \second{$\scriptstyle{\pm10}$}
                          & $\scriptstyle{\pm58}$
                          & $\scriptstyle{\pm9}$
                          & $\scriptstyle{2\%}$ \vspace{0.75ex} \\

    \texttt{finger,}        & $306$ & $884$ & $801$ & $923$ & \second{\bf{925}} & $922$ & \best{\bf{961}} & $+36$ \vspace{-0.75ex} \\    \texttt{spin}        
                          & $\scriptstyle{\pm12}$
                          & $\scriptstyle{\pm115}$
                          & $\scriptstyle{\pm65}$
                          & $\scriptstyle{\pm36}$
                          & \second{$\scriptstyle{\pm35}$}
                          & $\scriptstyle{\pm61}$
                          & \best{$\scriptstyle{\pm44}$}
                          & $\scriptstyle{4\%}$ \vspace{0.75ex} \\

    \texttt{walker,}        & $630$ & $955$ & $881$ & \second{\bf{959}} & $959$ & $952$ & \best{\bf{964}} & $+5$ \vspace{-0.75ex} \\    \texttt{stand}        
                          & $\scriptstyle{\pm224}$
                          & $\scriptstyle{\pm18}$
                          & $\scriptstyle{\pm51}$
                          & \second{$\scriptstyle{\pm5}$}
                          & $\scriptstyle{\pm6}$
                          & $\scriptstyle{\pm17}$
                          & \best{$\scriptstyle{\pm18}$}
                          & $\scriptstyle{1\%}$ \vspace{0.75ex} \\

    \texttt{walker,}        & $422$ & $827$ & $581$ & $753$ & $715$ & \second{\bf{876}} & \best{\bf{924}} & $+48$ \vspace{-0.75ex} \\    \texttt{walk}        
                          & $\scriptstyle{\pm42}$
                          & $\scriptstyle{\pm61}$
                          & $\scriptstyle{\pm129}$
                          & $\scriptstyle{\pm143}$
                          & $\scriptstyle{\pm74}$
                          & \second{$\scriptstyle{\pm45}$}
                          & \best{$\scriptstyle{\pm31}$}
                          & $\scriptstyle{5\%}$ \vspace{0.75ex} \\

    \texttt{cheetah,}        & $311$ & $333$ & $225$ & $300$ & $298$ & \second{\bf{343}} & \best{\bf{357}} & $+14$ \vspace{-0.75ex} \\    \texttt{run}        
                          & $\scriptstyle{\pm36}$
                          & $\scriptstyle{\pm43}$
                          & $\scriptstyle{\pm39}$
                          & $\scriptstyle{\pm37}$
                          & $\scriptstyle{\pm30}$
                          & \second{$\scriptstyle{\pm37}$}
                          & \best{$\scriptstyle{\pm25}$}
                          & $\scriptstyle{4\%}$ \vspace{0.75ex} \\



    \bottomrule
    \end{tabular}
    }
    \vspace{0.1in}
    \caption{train. \best{Red} indicates the best and \second{blue} indicates the second best. $\Delta=$ improvement of \dino over the second best.}
\end{table}

==> tables/dmc-gb-video-easy.tex <==

\begin{table}[t]
    \label{tab:dmc-all}
    \vspace{0.075in}
    \centering
    \resizebox{\tablesize\textwidth}{!}{%
    \begin{tabular}{cccccccccc}
    \toprule
    
    \bf{DMControl-GB}      & SAC & DrQ & SODA & SVEA    & SRM & SGQN & \textbf{SMG} & $\Delta$ \\
    (video easy)           &     &     &  &(overlay) &  (SAC) &   & (ours)       &          \\
    
    \midrule

    \texttt{cartpole,}        & $175$ & $606$ & $617$ & \second{\bf{718}} & $645$ & $717$ & \best{\bf{839}} & $+121$ \vspace{-0.75ex} \\    \texttt{swingup}        
                          & $\scriptstyle{\pm23}$
                          & $\scriptstyle{\pm31}$
                          & $\scriptstyle{\pm76}$
                          & \second{$\scriptstyle{\pm101}$}
                          & $\scriptstyle{\pm108}$
                          & $\scriptstyle{\pm77}$
                          & \best{$\scriptstyle{\pm16}$}
                          & $\scriptstyle{17\%}$ \vspace{0.75ex} \\

    \texttt{finger,}        & $171$ & $511$ & $615$ & $817$ & $642$ & \second{\bf{860}} & \best{\bf{952}} & $+92$ \vspace{-0.75ex} \\    \texttt{spin}        
                          & $\scriptstyle{\pm37}$
                          & $\scriptstyle{\pm192}$
                          & $\scriptstyle{\pm56}$
                          & $\scriptstyle{\pm94}$
                          & $\scriptstyle{\pm101}$
                          & \second{$\scriptstyle{\pm82}$}
                          & \best{$\scriptstyle{\pm48}$}
                          & $\scriptstyle{11\%}$ \vspace{0.75ex} \\

    \texttt{walker,}        & $484$ & $908$ & $924$ & $928$ & $947$ & \second{\bf{949}} & \best{\bf{961}} & $+12$ \vspace{-0.75ex} \\    \texttt{stand}        
                          & $\scriptstyle{\pm185}$
                          & $\scriptstyle{\pm38}$
                          & $\scriptstyle{\pm28}$
                          & $\scriptstyle{\pm50}$
                          & $\scriptstyle{\pm14}$
                          & \second{$\scriptstyle{\pm10}$}
                          & \best{$\scriptstyle{\pm19}$}
                          & $\scriptstyle{1\%}$ \vspace{0.75ex} \\

    \texttt{walker,}        & $325$ & $720$ & $518$ & $691$ & $662$ & \second{\bf{830}} & \best{\bf{904}} & $+74$ \vspace{-0.75ex} \\    \texttt{walk}        
                          & $\scriptstyle{\pm26}$
                          & $\scriptstyle{\pm69}$
                          & $\scriptstyle{\pm92}$
                          & $\scriptstyle{\pm120}$
                          & $\scriptstyle{\pm75}$
                          & \second{$\scriptstyle{\pm58}$}
                          & \best{$\scriptstyle{\pm34}$}
                          & $\scriptstyle{9\%}$ \vspace{0.75ex} \\

    \texttt{cheetah,}        & $179$ & $241$ & $215$ & $278$ & $253$ & \second{\bf{308}} & \best{\bf{348}} & $+40$ \vspace{-0.75ex} \\    \texttt{run}        
                          & $\scriptstyle{\pm65}$
                          & $\scriptstyle{\pm25}$
                          & $\scriptstyle{\pm15}$
                          & $\scriptstyle{\pm51}$
                          & $\scriptstyle{\pm27}$
                          & \second{$\scriptstyle{\pm34}$}
                          & \best{$\scriptstyle{\pm28}$}
                          & $\scriptstyle{13\%}$ \vspace{0.75ex} \\



    \bottomrule
    \end{tabular}
    }
    \vspace{0.1in}
    \caption{video easy. \best{Red} indicates the best and \second{blue} indicates the second best. $\Delta=$ improvement of \dino over the second best.}
\end{table}

==> tables/dmc-gb-video-hard.tex <==

\begin{table}[t]
    \label{tab:dmc-all}
    \vspace{0.075in}
    \centering
    \resizebox{\tablesize\textwidth}{!}{%
    \begin{tabular}{cccccccccc}
    \toprule
    
    \bf{DMControl-GB}      & SAC & DrQ & SODA & SVEA    & SRM & SGQN & \textbf{SMG} & $\Delta$ \\
    (video hard)           &     &     &  &(overlay) &  (SAC) &   & (ours)       &          \\
    
    \midrule

    \texttt{cartpole,}        & $156$ & $168$ & $346$ & $510$ & $254$ & \second{\bf{599}} & \best{\bf{764}} & $+165$ \vspace{-0.75ex} \\    \texttt{swingup}        
                          & $\scriptstyle{\pm16}$
                          & $\scriptstyle{\pm35}$
                          & $\scriptstyle{\pm59}$
                          & $\scriptstyle{\pm177}$
                          & $\scriptstyle{\pm69}$
                          & \second{$\scriptstyle{\pm112}$}
                          & \best{$\scriptstyle{\pm32}$}
                          & $\scriptstyle{28\%}$ \vspace{0.75ex} \\

    \texttt{finger,}        & $22$ & $54$ & $310$ & $353$ & $131$ & \second{\bf{710}} & \best{\bf{910}} & $+200$ \vspace{-0.75ex} \\    \texttt{spin}        
                          & $\scriptstyle{\pm10}$
                          & $\scriptstyle{\pm44}$
                          & $\scriptstyle{\pm72}$
                          & $\scriptstyle{\pm71}$
                          & $\scriptstyle{\pm89}$
                          & \second{$\scriptstyle{\pm159}$}
                          & \best{$\scriptstyle{\pm61}$}
                          & $\scriptstyle{28\%}$ \vspace{0.75ex} \\

    \texttt{walker,}        & $212$ & $278$ & $406$ & $814$ & $558$ & \second{\bf{870}} & \best{\bf{955}} & $+85$ \vspace{-0.75ex} \\    \texttt{stand}        
                          & $\scriptstyle{\pm41}$
                          & $\scriptstyle{\pm79}$
                          & $\scriptstyle{\pm68}$
                          & $\scriptstyle{\pm57}$
                          & $\scriptstyle{\pm139}$
                          & \second{$\scriptstyle{\pm78}$}
                          & \best{$\scriptstyle{\pm9}$}
                          & $\scriptstyle{10\%}$ \vspace{0.75ex} \\

    \texttt{walker,}        & $132$ & $110$ & $175$ & $348$ & $165$ & \second{\bf{634}} & \best{\bf{814}} & $+180$ \vspace{-0.75ex} \\    \texttt{walk}        
                          & $\scriptstyle{\pm26}$
                          & $\scriptstyle{\pm33}$
                          & $\scriptstyle{\pm31}$
                          & $\scriptstyle{\pm80}$
                          & $\scriptstyle{\pm99}$
                          & \second{$\scriptstyle{\pm136}$}
                          & \best{$\scriptstyle{\pm51}$}
                          & $\scriptstyle{28\%}$ \vspace{0.75ex} \\

    \texttt{cheetah,}        & $56$ & $38$ & $118$ & $105$ & $87$ & \second{\bf{135}} & \best{\bf{303}} & $+168$ \vspace{-0.75ex} \\    \texttt{run}        
                          & $\scriptstyle{\pm30}$
                          & $\scriptstyle{\pm26}$
                          & $\scriptstyle{\pm40}$
                          & $\scriptstyle{\pm13}$
                          & $\scriptstyle{\pm24}$
                          & \second{$\scriptstyle{\pm44}$}
                          & \best{$\scriptstyle{\pm46}$}
                          & $\scriptstyle{124\%}$ \vspace{0.75ex} \\



    \bottomrule
    \end{tabular}
    }
    \vspace{0.1in}
    \caption{video hard. \best{Red} indicates the best and \second{blue} indicates the second best. $\Delta=$ improvement of \dino over the second best.}
\end{table}

==> tables/rebuttal.tex <==

\begin{table}[ht]
    \caption{Additional results with more baselines and ablation study.}
    \label{table:dmc-video}
    \vspace{0.1in}
    \centering
    \resizebox{\tablesize\textwidth}{!}{%
    \begin{tabular}{cccccccccc}
    \toprule
    
    \bf{DMControl}         & SAC & SVEA     & SGQN & TIA & SAM-G    & \textbf{SMG} & \textbf{SMG} & \textbf{SMG} & $\Delta$  \\
    (\textit{video-hard})  &     &(overlay) &      &     & (PIE-G)  &  ($\lambda_{\text{fore}}=1$)  &(SAC)        &     (SVEA)   &           \\
    
    \midrule

    \texttt{cartpole,}    & $156$ 
                          & $510$ 
                          & $599$ 
                          & $52$ % TIA
                          & \second{\bf{653}} % SAM-G
                          & $670$ (-12\%)
                          & \best{\bf{764}}
                          & $750$ % SMG(SVEA)
                          & $+111$ \vspace{-0.75ex} \\    
    \texttt{swingup}        
                          & $\scriptstyle{\pm16}$  
                          & $\scriptstyle{\pm177}$ 
                          & $\scriptstyle{\pm112}$
                          & $\scriptstyle{\pm32}$  % TIA
                          & \second{$\scriptstyle{\pm58}$}  % SAM-G
                          & $\scriptstyle{\pm104}$
                          & \best{$\scriptstyle{\pm104}$} %SMG(SAC)
                          & $\scriptstyle{\pm33}$  % SMG(SVEA)
                          & $\scriptstyle{28\%}$ \vspace{0.75ex} \\

    \texttt{finger,}      & $22$ 
                          & $353$ 
                          & $710$
                          & $64$ % TIA
                          & \second{\second{\bf{908}}} % SAM-G
                          & $706$ (-22\%)
                          & \best{\bf{910}}
                          & $905$ % SMG(SVEA)
                          & $+2$ \vspace{-0.75ex} \\    
    \texttt{spin}        
                          & $\scriptstyle{\pm10}$
                          & $\scriptstyle{\pm71}$
                          & $\scriptstyle{\pm159}$
                          & $\scriptstyle{\pm56}$  % TIA
                          & $\scriptstyle{\pm66}$  % SAM-G
                          & $\scriptstyle{\pm127}$
                          & \best{$\scriptstyle{\pm61}$}
                          & $\scriptstyle{\pm69}$  % SMG(SVEA)
                          & $\scriptstyle{0\%}$ \vspace{0.75ex} \\

    \texttt{walker,}      & $212$ 
                          & $814$ 
                          & $870$
                          & $271$ % TIA
                          & \best{\bf{964}} % SAM-G
                          & $876$ (-8\%)
                          & $955$
                          & \second{\bf{962}} % SMG(SVEA) 
                          & $-2$ \vspace{-0.75ex} \\    
    \texttt{stand}        
                          & $\scriptstyle{\pm41}$
                          & $\scriptstyle{\pm57}$
                          & $\scriptstyle{\pm78}$
                          & $\scriptstyle{\pm56}$  % TIA
                          & \best{$\scriptstyle{\pm4}$}  % SAM-G
                          & $\scriptstyle{\pm44}$
                          & $\scriptstyle{\pm9}$
                          & \second{$\scriptstyle{\pm62}$}  % SMG(SVEA)
                          & $\scriptstyle{0\%}$ \vspace{0.75ex} \\

    \texttt{walker,}      & $132$ 
                          & $348$ 
                          & $634$
                          & $109$ % TIA
                          & \best{\bf{857}} % SAM-G
                          & $805$ (-1\%)
                          & $814$
                          & \second{\bf{837}} % SMG(SVEA) 
                          & $-20$ \vspace{-0.75ex} \\    
    \texttt{walk}        
                          & $\scriptstyle{\pm26}$
                          & $\scriptstyle{\pm80}$
                          & $\scriptstyle{\pm136}$
                          & $\scriptstyle{\pm15}$  % TIA
                          & \best{$\scriptstyle{\pm31}$}  % SAM-G
                          & $\scriptstyle{\pm53}$
                          & $\scriptstyle{\pm51}$
                          & \second{$\scriptstyle{\pm45}$}  % SMG(SVEA)
                          & $\scriptstyle{2\%}$ \vspace{0.75ex} \\

    \texttt{cheetah,}     & $56$ 
                          & $105$ 
                          & $135$
                          & $19$ % TIA
                          & \second{\bf{327}} % SAM-G 
                          & $265$ (-13\%)
                          & $303$
                          & \best{\bf{330}} % SMG(SVEA) 
                          & $+3$ \vspace{-0.75ex} \\    
    \texttt{run}        
                          & $\scriptstyle{\pm30}$
                          & $\scriptstyle{\pm13}$
                          & $\scriptstyle{\pm44}$
                          & $\scriptstyle{\pm9}$  % TIA
                          & \second{$\scriptstyle{\pm11}$}  % SAM-G
                          & $\scriptstyle{\pm18}$
                          & $\scriptstyle{\pm46}$
                          & \best{$\scriptstyle{\pm32}$}  % SMG(SVEA)
                          & $\scriptstyle{1\%}$ \vspace{0.75ex} \\



    \midrule

    \toprule
    
    \bf{Robtic-Manipulation}  & SAC & SVEA     & SGQN & TIA & SAM-G    & \textbf{SMG} & \textbf{SMG} & \textbf{SMG} & $\Delta$  \\
    (\textit{test-1})          &     &(overlay) &      &     & (PIE-G)  &  ($\lambda_{\text{fore}}=1$)  &(SAC)        &     (SVEA)   &           \\
    
    \midrule

    \texttt{reach}
                   & $-16$
                   & $-22$
                   & \second{\bf{19}}
                   & $-9$
                   & -
                   & $26$ (-13\%)
                   & $30$
                   & \best{\bf{31}}
                   & $+12$ \vspace{-0.75ex} \\
    
                   & $\scriptstyle{\pm33}$
                   & $\scriptstyle{\pm16}$
                   & \second{$\scriptstyle{\pm13}$}
                   & $\scriptstyle{\pm27}$
                   & -
                   & $\scriptstyle{\pm3}$
                   & $\scriptstyle{\pm1}$
                   & \best{$\scriptstyle{\pm5}$}
                   & $\scriptstyle{39\%}$ \vspace{0.75ex} \\
    
    \texttt{peg-in-box}
                   & $-33$
                   & $-18$
                   & $-67$
                   & \second{\bf{86}}
                   & -
                   & $193$ (-19\%)
                   & \best{\bf{237}}
                   & $220$
                   & $+151$ \vspace{-0.75ex} \\
    
                   & $\scriptstyle{\pm25}$
                   & $\scriptstyle{\pm59}$
                   & $\scriptstyle{\pm28}$
                   & \second{$\scriptstyle{\pm113}$}
                   & -
                   & $\scriptstyle{\pm25}$
                   & \best{$\scriptstyle{\pm18}$}
                   & $\scriptstyle{\pm31}$
                   & $\scriptstyle{64\%}$ \vspace{0.75ex} \\

    \bottomrule


    \end{tabular}
    }
\end{table}
